Technical Report: Design, Implementation and Deployment of Intermittency-aware Cellular Edge Services for Rural areas

Rural areas continue to be plagued by limited data connectivity due to poor and unreliable power infrastructure, poor backhaul connectivity and lack of economic incentives for telecom providers. These factors continue to be an impediment to providing reliable, highly available and bandwidth intensive mobile services and applications to function well in such contexts. This paper presents the design, implementation and deployment of GreenLinks, a new ground-up platform that enables intermittency-aware, reliable and available cellular services and application support in rural contexts under extreme operational environments with limited power and no existing cellular coverage. Unlike the conventional monolithic cellular network architecture, GreenLinks enables a distributed (and potentially disjoint) collection of open, programmable cellular base stations to offer a gamut of both conventional cellular services and new forms of distributed edge services. GreenLinks offers new application primitives to support different types of intermittency-aware distributed mobile edge services including P2P transactions, voice-based social media applications, and distributed mobile sensing applications. Using a participatory sensing white spaces approach, a GreenLinks base stati

==> Not Needed?/architecture.tex <==
\section{VC-ISP Architecture}


\begin{figure*}
\centering
	\includegraphics[width=0.8\textwidth]{figures/SystemArch.jpg}
\caption{Architecture of VC-ISP}
\label{fig:systemArch}
\end{figure*}


Figure~\ref{fig:systemArch} illustrates the elaborate network structure and the system architecture of a VC-ISP. A VC-ISP should be viewed a cellular network that extends coverage to previously uncovered area(s). As mentioned earlier, VC-ISP builds upon two key technological ingredients: (a) software defined cellular network nodes; (b) stable backhauls for reliable backwards communication. The rural areas don't have many stable options for connecting with the rest of the world. The more isolated areas have no way to connect other then satellite communication or long range wifi. While many areas have weak cellular signals that are sometimes leveraged by using repeaters~\cite{http://vimeo.com/78562876}. This is often considered a cheapest solution for the residents of hundreds of square Kilometres who are at the border of connectivity corridor. We see our VC-ISP implementation as working using one or multiple non-homogeneous backhaul connectivity solutions available in the region, which can be fiber connectivity, telephone or power lines or can leverage recent advances in high speed mobile backhaul connectivity~\cite{kumunetworks,tarana}.  

The basic building block of VC-ISP is a {\em node} which represents a software-defined cell tower which is low power and completely programmable. The node is connected to the internet by means of synthetic stable link which can leverage multiple low-bandwidth links. Any node that is not connected to the IP backbone has a backhaul link to other nodes in the network and can eventually connect to one or more {\em gateway} nodes. A {\em zone} represents a collection of
inter-connected nodes with backhaul links within a geographic locality with one or more gateway nodes.

As shown in Figure~\ref{fig:systemArch}, the VC-ISP network is composed of multiple {\em zones} each with its own gateway nodes and a cloud based infrastructure that aids in interconnecting the nodes into a cohesive virtual cell architecture. The cloud infrastructure of
VC-ISP has 3 key components: (a) forwarding nodes; (b) lookup and messaging servers; (c) PBX endpoints. Gateway nodes that are not behind NATs can act as forwarding nodes for their zones and gateway
nodes that are behind NATs require a cloud-based forwarding node with
a public IP address. These nodes are responsible for forwarding
traffic either between zones or between zones and the conventional
cellular network through PBX servers, which help in interfacing with
the cellular network. The lookup and messaging servers play a critical
role in enabling VC-ISP to offer a variety of intermittency-aware
services across zones and also provide compatibility with the same
services offered by a traditional cellular network. 

\subsection{BTS Nodes} Every node in VC-ISP runs the OpenBTS platform
which offers a software-defined cellular services. The BTS nodes are attached to a local machine which we refer to as a \textit{local server} which runs the local component of various services.  Each BTS node is responsible for providing basic cellular services(calls, sms and data) and other interactive services built on top of cellular services to users directly connected to them. While the local server next to the BTS node makes sure that they can work independently in the face of failures to provide local services while also having the capability to store messages to later sync up with gateway node and the rest of the nodes after recovery from intermittent node failures.  

It is important to mention that every node has a low energy profile which makes it a suitable candidate for use with low cost renewable energy solutions.  The core part of each node is the software platform that enables us to provide an array of services in a distributed manner where there is very less dependency between the devices located at different geographic locations in the network. This helps us build a highly available local network because in case of a partition, the
connected nodes form a network among them that enables mobile devices within a connected region to lookup and reach each other. As shown in Zone B in Figure~\ref{fig:systemArch}; VC-ISP provides intermittency-aware messaging services to devices which are not in the connected region. This is vital for enhancing availability of services in lieu of intermittent failures.

\subsection{Zones, Devices, Lookup and Routing} Each zone is maintained as a private network that provides coverage to a geographic locality where each BTS
node is allocated a sub-prefix in the private network range. Each zone
operates independently and communicates with other zones using the
forwarding nodes and the lookup and messaging servers.  Different
devices can connect the GreenLinks system. Each device needs to have a
unique identifier and a unique secret associated with that identifier
to authenticate to GreenLinks, upon which each device is associated
with an address that is directly reachable within a zone. When a
device joins GreenLinks, it registers with the local BTS node within a
zone and its identity and its allocated address (by the local BTS) are
disseminated to the lookup system both within the zone and the lookup
servers in the cloud.  GreenLinks uses a distributed naming/addressing
protocol to resolve device names into zone-level addresses. An address
of a device in GreenLinks refer to a (zone, private IP address)
mapping. When a device initiates a lookup for a name, the name is
first resolved at the intra-zone level, then at the inter-zone level
(if intra-zone is unsuccessful) and finally using the conventional
cellular level (if inter-zone is unsuccessful).
GreenLinks supports three types of routes: intra-zone routes,
inter-zone routes, zone-PBX routes.  Within each
zone, GreenLinks uses an energy aware routing protocol that enables
every BTS node to reach a gateway node and other BTS nodes within the
zone. Since each BTS operates a separate sub-prefix, the address to
BTS mapping is straight-forward. An inter-zone routing path is a
simple amalgamation of 2 intra-zone paths from/to the gateway nodes
and a direct IP path between the forwarding nodes of the zones. The
gateway/forwarding nodes also act as NAT address translators for
internal IP addresses. The zone-PBX routes are for routing voice calls to the
cellular network using the closest PBX server.




==> Not Needed?/implementation.tex <==
\section{Implimentation and Deployment}



==> Not Needed?/primitives.tex <==
\section{Programmable Platform and service primitives}

\begin{figure}
\centering

        \includegraphics[scale=0.25]{dht.pdf}

\caption{Architecture picture for a more scalable VCN architecture with multiple nodes connected to multiple cloud servers that form a DHT based mechanism for storage and satisfying other requests}
\label{dht}
\end{figure}


In this section we try to highlight the routing mechanism and primitives that enable us to leverage the hardware platform to provide a programmable framework for edge services. To our knowledge this is the first paper evaluates deploying an array of services next to a cellular base station using high level primitives on a programmable platform. 

Our first guiding principle was introducing a clear separation in the server 
side functionality and moving most of the computation part of the applications 
to a local server while leave the long term storage and facilitation 
part in the cloud. 
Our next guiding principle was to develop high level abstraction for 
low level routing, for this we tried to build a simple application 
independent API to handle low level routing between different software 
components of OpenBTS, PBX, local and cloud servers. 
The software platform of Ubuntu provides ease of doing content 
interception and routing of all the traffic in an online manner 
to the appropriate content handling component. 
Having a fully customizable operating systems we had the flexibility to 
use new ways to do various tasks which are best in small packet regimes.  

We start by describing Identity management in our system. Which is the 
bases of device to device communication. We describe two different architectures 
for identity management, namely client-server model and dht-model. For naming and addressing in our 3-node deployment we used the client-server model while we 
envision using the dht-model for scalability when the number of nodes and number 
of users in the network increases. We evaluate DHT model using large scale 
simulators. 

\subsection{Identity Management}
The goal of identity management is to issue new identities to new users who join the network and to diseminate the information in network so that communication 
can be enabled between devices inside and outside our network. 
%While \name is itself a cellular network that issues its own identity. 
\name issues two kinds of identities: namely locally accessable and globally accessable identities. As the name suggests, local identities are only available 
inside the network while global identities make it possible for devices 
from outside the network to connect with the devices inside the network. 
Local identities in the network are quite flexible and we can accommodate commonly used identities like skype names and google talk ids. 
This is because we use OpenBTS software, which is open-source and modular. 
Identity management layer enables applications to route messages in a 
seamless manner.   

%Apart from using multiple different identities in the system, We also provide a vpn-based solution for connecting nodes that are behind NATs so that the users on one geographic locality can conveniently reach the other locality. A vpn-based approach works better than standard VOIP solutions for machines behind NATs. In the rest of the section we give an overview of the naming and addressing layer of VC-ISP and describe the mechanism used for interoperability of users inside a single VC-ISP. 

%The Identity management layer of \name aims to allow different types of end-devices to seamlessly join the network. 
%It also allows devices to use their conventional names (mobile phone numbers, Skype user identities) 
%and enables them to discover other devices within the network. The \name design achieves this goal without the need for any modification to the end-devices. All entities in the \name architecture play crucial roles for the implementation of this layer in a distributed fashion. 

As mentioned earlier we design and test two different identity management models. 
In the simulation environment implementation we use the DHT-based model, 
while for our practical 3-node deployment we use a simple server-client model. 
The reason for this distinction is that a DHT-based approach is not required at a 3-node scale, 
while simulation environment tries to evaluate scalability of \name.  
We explain how both these models of naming/addressing work. 

\subsubsection{Server-Client Model}
In the server-client identity model, there is a central entity that issues global and local identity. If a new user comes to any node, the request is routed to the central server and the identity of that user is issued by the server. The server keeps record of each identity that was issued to each node. In addition it records the IMSI number of the SIM card to which the identity was issued. Hence if the user moves to a different node, the server still knows that an identity has been issued and only the address of the user needs to be updated.

User is allowed to choose its own identity, which can be its skype number or some other number that he likes. But that identity will only be accessible directly from another users on the \name network. In order to enable outside users(that do not belong to \name) to reach this device a second identity is required which is reachable from any node. For this we issue global identities using a VOIP service which sends the calls and messages from outside users to our cloud server which in turn sends them to the node where user exists. 

This server-client model can have a hierarchy where a server keeps track of all the identities of its children. Each zone(geographic locality) has its own server which issues and keeps track of all the users in that particular zone. As it can be imagined this gives rise to a 3 layer system. The first layer consists of the one central root server and the second layer consists of all the zone level servers while the third layer is comprised of all the nodes in the zones. This kind of a setup is simple and easy to incrementally build but it is not very scalable. If the number of users are oddly distributed among zones the zone servers can become a bottleneck for the zone. If the number of users is evenly distributed, even then the root server can become a bottleneck for users trying to connect with users in other zones. 
%It can be argued that we can have multiple virtual servers in root layer instead of one server like DNS but the odd distribution among zones can still not be handled. Therefore we look at a DHT based approach for naming and addressing beyond a point where users cannot be handled by a single node. 
   
 
\subsubsection{DHT Model}
To overcome the scalability limitations of client-server model we propose usage of a DHT based naming model. We envision a more scalable architecture if there are multiple sites in different regions around the world. Figure~\ref{dht} shows the architecture we envision where a BTS nodes connects to the cloud controller physically closer to it and thus there are multiple cloud servers. All the cloud controllers are located in data centers and have high bandwidth links to other cloud controllers. These cloud controllers form a distributed hash table for managing identities and application level processing among them in order to deal with failures and to provide faster access even when there is a skew in users between different nodes. Having multiple distributed central servers helps evenly divide the storage and processing duties of the cloud controllers that are dealing with too much traffic. The model is inspired from the DHT based design of WiRE~\cite{wire} and SEATTLE\cite{seattle}.

Given an arbitrary client initially connects with a BTS node $b$ which 
is connected to a cloud server $k$ (the cloud server that is nearest) the client. 
The local server sends the IMSI number(identifier of SIM card) to the cloud 
server $k$. Depending on if user wants a global identity or local identity, 
an identity is issued by the cloud server $k$. 
While a response is sent back to the client telling him 
his identity, the next step is to identify the \textit{resolver} node for 
the identity pertaining to this client. The resolver is the cloud server that 
is responsible for storing any data related to this identity. This includes all 
data related to identity and applcations being used by the identity. 


Let $m$ be the mobile device identity issued and let $G$ be the list 
of all cloud server nodes. Then for every node $x \in G$, $k$ calculates $H(x)-H(m)$ where H is the hash function. Resolver is defined as the node $x^*$ that minimizes $H(x)-H(m)$. The resolver node is the node which maintains the information about gateway node of the zone in which $m$ is present. This DHT based approach solves the problem of uneven distribution of users across geographic localities discussed in the last section but there is extra overhead for lookup for each query. 

\begin{comment}
\subsection{Interoperability}

A big part of VC-ISP identity management is interoperability among different zones of the VC-ISP. The VC-ISP naming and addressing layer facilitates interoperability of identities between zones because of the way identities are issued. The identity issuing in both the models discussed above is done by a single server. Therefore it is easy to see if an identity has been issued to a particular user before or not. In our system we assume that each user connects with a single SIM card when he moves accross zones. Therefore if an old IMSI asks for a new ID or simply joins the network, the network can know from the identity issuing server can identify it as an old user. 

Interoperability within a particular zone is as important as interoperability between the different zones of a VC-ISP. For interoperability between nodes that share range we use the mechanism for handover used in OpenBTS\cite{http://wush.net/trac/rangepublic/wiki/Handover-quickstart} based base stations and it suffices to achieve interoperability in the area with a uniform coverage by VC-ISP having multiple base stations with overlapping ranges. However if nodes in a zone do not overlap with each other and user appears in a second base station in the zone then the identity issuing authority has to be updated and the address of the identity changed and new address disseminated using the naming/addressing model that is being used. 

We provide two different mechanism for validating the user at a new address. The first method is triggered by the system itself. A base station upon seeing an unauthorized user making a call or SMS executes the procedure for discovering if the user is already registered from a different base station. In case a user exists, the user is validated and its address is updated in the address lookup tables. If there are any messages for him that were not able to reach him because of his absence from his previous known address, they are delivered to him. In the second method we provide a sms short code where user sends a free sms to validate itself and this way the system updates its lookup tables. 
\end{comment}

\subsection{Service Primitives}
We build a few application independent service primitives by leveraging the identity management layer defined in the last section. These primitives are used to manage and develop several applications discussed in future sections. It is important to highlight that these primitives are very generic and were developed keeping in mind the architecture of applications required by developing countries. 

First primitive is \texttt{POST(Identity i, Type t, Data d)} is the abstraction that is used to send data from local server to cloud server is a \textit{lazy} manner. This means that the data may not be immediately sent after the primitive is executed but the server determines the right order to send the data from local to cloud server based on bandwidth availability and other requests in the queue. Depending on the application type t, data can be prioritized. Second primitive is \texttt{GET(Identity i)} which is used by the local server to fetch data pertaining addressed to a particular identity. For instance if a user x left a message for user i, the local server for user i will fetch that message using the GET(i) request given above. This primitive is important in getting messages left by others for a particular device. This primitive is not executed in a lazy manner.  Third primitive is \texttt{Search(Type t, Data d)} which is used by the local server to search for data of a particular application type t. This command is similar to GET and returns one or more data points based on search from the cloud data store. Fourth primitive is \texttt{Send(Type t, Data d, To j)} and is used to send data directly from the cloud server to a user j on one of the local servers, this operation is done in a \textit{lazy} manner. 

These primitives hide the data the internal implementation of naming and addressing and enable complex applications to be built on top. For example if we want to build a voice messaging application, it can be built using the three primitives given above. An IVR system running on the local server enables recording of messages, in the next step user gives the identity of the user it wants to send the voice message to. On the backend the application uses the POST and SEND primitives to send the message from the sender to receiver. These primitives are extremely similar to a distributed file system and in some sense this is a distributed file system but what is novel about this is the queuing mechanism in place to work with the limited bandwidth between local and cloud server. 





==> Not Needed?/program.tex <==
\section{Programmable Platform}
In this section we try to highlight the guiding principles that enabled us to leverage the hardware platform to provide a programmable framework for edge services. To our knowledge this is the first paper evaluates deploying an array of services next to a cellular base station. 

Our first guiding principle was introducing a clear separation in the server side functionality and moving most of the computation part of the applications to a local server while leave the long term storage part in the cloud. Our next guiding principle was to develop high level abstraction for low level routing, for this we tried to build a simple application based API to handle low level routing between different software components of OpenBTS, PBX and local cluster. We also did content interception and routed all the traffic in an online manner to the appropriate content handling component. Having a fully customizable operating systems we had the flexibility to device new ways to do various tasks which are best in small packet regimes.  

\subsection{Heavier local server, lazy cloud synchronization}
The server side of most of the applications are located in the cloud component and most of the cloud infrastructure is hosted in developing countries. In our platform one of the most important contributions is that we reduce the amount of cloud component and increase the size of local component. In particular we try to move the processing(computation-intensive) part of the server functionality to a local server connected to a base station. This helps reduce latency in server response and also helps in reducing the bandwidth consumption between the server and client resulting is saving revenue because bandwidth is expensive in developing countries. 

It can be argued that this migration will lead to other problems like scalability and ease of management that comes with having the complete application in cloud. But we show that the applications at a base station level don't scale to millions of users and are able to work with a lazy data synchronization with the light weight cloud component. Furthermore this approach leads to limited need of data transmission between the local server and cloud, which can be easily upper bounded and thus the cost can more predictable and manageable. 

Having a heavier local server has a major advantage in view of unstable backhauls available in the rural areas of developing world. Most of the commercial cellular towers need to connect to the service gateways for simple tasks like validating users and local calls. But with having a local server, a cell tower can not only continue to perform these basic tasks but advanced tasks like IVR based applications and even web surfing of cached webpages in the eventuality of a broken backhaul link. 

It can be argued that having a server at each base station will be an overkill because in lower load timings the server will not be performing any tasks but will be idle. While this is true the cellular towers in the rural areas are mostly not required in night times and are shut down to save power. In addition to this, a local server at a base station will have a lower energy profile as compared to supporting the full application in the cloud in terms of cooling apparatus required. We show in the deployment and evaluation we were able to support the base station and the associated server with a 1KW solar setup in rural Ghana.



\subsection{High level abstraction for low level routing}
Routing between different components of OpenBTS, Freeswitch and the local server is critical for any framework to build applications. There is a wide variety of packet traffic that is routed, for example the traffic between PBX and local server can be HTTP, TCP, SIP or FTP depending on the application. We build an abstraction on top of iptables to install appropriate rules depending on a configuration file. This mechanism helps the user in generating and managing the kernel routing tables using a high level substrate. 

The design of the software platform is very modular. The components providing different services can be replaced by efficient components while the underlying routing remains the same because the routing management layer is independent of components and gives the users an abstraction for interception. 

For example any sms based application requires the sms directed to a particular short code to be routed to a server running on a particular port in the server machine. The application expects to know the identity of the user who sent that sms and a callback URL where it can post the message back after processing. Instead of configuring the PBX, POST parameters and callback URL manually, all the details are given in the form of a one line instruction in the configuration file. \texttt{sms(shortCode,protocol,portNumber,dataMethod)} which suggests that a protocol(e.g. TCP, HTTP) is running on \texttt{port=portNumber} and it expects data of type \texttt{dataMethod}(e.g. POST, GET, CSV, JSON) data. 

In a similar manner the web caching, IVR and sensing applications can be implemented with one line instructions. We built the routing API on top of iptables and freeswitch PBX to provide an array of different services. The framework helps us deploy sms based, IVR based, caching based and sensor apps(mobile data collection) apps in an easy manner. To our knowledge this is the first framework that allows building applications so close to the base station. 

It is pertinent to realize that users are kept unaware of the backend functionality that is being employed. So in the example of a web caching server Instead of asking the users to each configure their mobile devices to access web through the cache, we isolate all the web request and route it through a caching server using iptable rules. Similarly in case of sms and IVR applications users are only exposed a mobile short code of a service. In case of IVR users can be given a SIP identity of the IVR application to directly call that application but we hide that detail and use content interception to identify the appropriate destination based on the configuration file. 

\subsection{Flexibility for newer solution}
This section gives a comparison with conventional cellular networks. For routing and fine-grained packet processing, conventional cellular providers rely on specialized and proprietary devices, namely: Serving Gateways (S-GWs) and Packet data network Gateways (P-GWs). S-GWs are responsible for providing seamless mobility while P-GWs centralize most network functions like content filtering, traffic optimization, firewalls, and lawful intercept [4]. P-GWs sit at the boundary of the cellular network and the Internet. In our case our local server becomes the P-GW and does all the packet processing and routing required. 

In commercial cellular networks centralizing nearly all important functionalities in the P-GWs makes cellular core networks remarkably inefficient, complex, and inflexible \cite{elby2012carrier,kim} for two major reasons. First, cellular core networks must forward all traffic through the P-GWs—including device-to-device traffic and local content distribution network services. This increases the network latency and congestion and makes a single base station dependent on an array of different hardware to provide simple functionalities. Second, since P-GWs are not modular, carriers have to take what is available from hardware providers and they don't have a chance to choose between different capabilities from different providers to mix and match; when a function is not available, carriers have no choice but to replace the P-GWs—even if they are sufficient for most purposes~\cite{chiosi2012network,jin2013softcell}.

In case of an OpenBTS based cell, various components are brought together at the cell. All of the P-GW functionality is performed by the server next to the base station. This gives us a unique opportunity to impliment newer methods for different tasks in the mini network between the base station and local server. For example, we can have our own alternative to FTP for sensor applications because FTP connections timeout in small packet regimes and our base station only supports GPRS connections. 
 

==> content/1-intro.tex <==
\section{Introduction}

Cellular networks have achieved significant penetration levels in developing regions in the past decade. However, much of this growth has been predominantly urban-centric with relatively low rural presence~\cite{wildnet,2P,litmac,delaycheck,beyond,heimerl}.  The existing cellular connectivity model is not economically viable for rural settings due to a multitude of fundamental challenges in rural contexts:

{\bf Power:} Rural regions lack stable and reliable grid power. Cellular networks are inherently power hungry in rural settings (to blanket large areas) and often rely on diesel-powered generators for power, which is a highly expensive proposition~\cite{ahmad:ictd15}. Staggeringly, the second largest consumer of oil in India is the telecommunications industry~\cite{trai}.

{\bf Lack of Financial Incentives:} While cellular networks incur high capital and operational expenses, the demand often does not match the
cost due to low user-densities and low purchasing power. For years, low demand and high usage costs have been locked in a vicious cycle.
Recently, Bharti Airtel and Reliance Communications, two of the largest cellular service providers in India, announced their interest to pull out of rural markets due to unfavorable economics~\cite{bhartiairtel}.

{\bf Lack of reliable backhauls and data services:} Data connectivity is largely absent in rural settings; where connectivity is available, options are generally restricted to voice and SMS messages~\cite{hermes, smarttrack}. Backhaul This has been a roadblock to the introduction of new data-driven services.

{\bf Reliability:} Maintenance of rural wireless networks is very hard due to a myriad of reliability problems, power-related problems and lack of local expertise to fix them. Lack of clean power is known to trigger frequent device failures in rural networks~\cite{beyond}.

\textcolor{red}{Talal: It is pertinent to mention the rigidity of the cellular architecture here. In particular we need to focus on the identity management in conventional cellular networks so that we can make a strong case of our new identity management (we have a whole section on this). Also we need to mention the architecture of cellular network because we have to talk how our services are deployed close to the edge.}
 
%Limited bandwidth is another issue faced by most rural areas in bandwidth. The only internet available in most of the rural areas is mobile internet and because of low-population density the commercial cellular providers have limited incentive to provide high quality internet. Furthermore studies have shown that people are careful of data usage because of the cost despite high interest. Most of the mobile applications popular among people in these areas are data-efficient and contribute meaningfully to their life~\cite{dalvitdata}. This highlights two important needs of such communities. Less bandwidth consumption and need for useful relevant services. 


%More recently there have been community collaborated efforts by researchers in this area\cite{kurtis_ictd,zheleva}. These initiatives have helped provide means to make cellualar network available and affordable for many people in isolated settings. While this is a decent start, we believe that the problem is deeper and a good solution has to cover all bases of the problem. A good solution does not only have to be cheap, convenient and easy to use it has to provide a better interface for management of larger distributed deployments of these cellular units while providing services in a sustainable manner to inadequately connected communities. 

In this paper, we present the design, implementation and deployment of {\em Virtual Cellular ISPs (VC-ISP)}, a new ground-up cellular network
architecture that enables third-party vendors to offer cellular coverage and mobile services in rural areas in an extensible manner. The basic building of the VC-ISP network architecture is a Virtual Cellular Node (VCN) which are open, programmable cellular base station platforms~\cite{range, openbts, openradio, softcell} that enable easy deployment of low-power software defined base stations that function effectively over an IP backplane.  Given that VC-ISPs are designed for areas with limited cellular coverage, the second building block of the VC-ISP model is the use of highly directional backhauls to extend backhaul connectivity to the VCNs; here, we show how one can easily design such backhauls to achieve reliable, high bandwidth IP connectivity to VCNs even in areas with relatively negligible coverage.

The VC-ISP network architecture builds upon on existing work on community cellular networks\cite{kurtis_ictd,zheleva,anand,rhizo} which can be viewed as stand-alone installations of virtual cellular nodes. In the VC-ISP architecture, we aim to address the following question: {\em How do we enable a distributed and potentially disjoint collection of open, programmable cellular base stations to act in unison as a single virtual cellular ISP?}.  Given the lack of incentives for conventional cellular providers to provide rural connectivity, the VC-ISP model empowers third-party providers to act as cellular providers and offer the entire gamut of conventional cellular services including voice, messaging and data.  In addition,
due to the programmable nature of individual VCNs, we show how VC-ISPs can provide new forms of distributed mobile edge services where
computation, storage and application state can be moved to the mobile edge. 

The design of VC-ISP addresses the following key research challenges:

{\em 1. White Spaces:} VC-ISPs reuses spectrum allocated to cellular operators using a participatory sensing white spaces approach to determine channels and detect conflicts from conventional cellular operators. The white spaces approach also enables co-existence across competing VC-ISPs in a region.\textcolor{red}{Talal: if we claim that VC-ISPs compete we have to provide \\a) an algorithm and workable logistics with sharing of sensing data in a database and \\b) supported evaluation for this. \\ we currently don't have both these things. This is potentially one area we can go deeper into. }

{\em 2. Reliable Backhauls:} In areas which are at the boundaries of conventional cellular coverage (where signals are negligible but existent),VC-ISPs can establish reliable backhauls that can provide several Mbps cellular backhaul bandwidth in areas with near-zero coverage using parallel directionally boosted data links to conventional cell towers. \textcolor{red}{Talal: We don't have any eval to support this particular aspect. I can remember we boosted two links at the same time. The numbers we have eval for a gain in single link. What can we realistically do to prove this? I don't think simulations will be useful at all.  We can try to get a multi path tcp thing running, but that requires compiling the multi path tcp kernel and then showing the real throughput. Will this make it a worthy contribution? Part of me tells me people will dismiss it as just a proof of concept because hardware and software are both already there and we don't do anything.}

{\em 3. Identity Management:} To provide Internet and conventional cellular services, VC-ISP supports an identity management layer that {\st{allows different types of authorized end-devices (mobile phones, WiFi devices) to join the network while using their conventional names (mobile phone numbers, WiFi-network user identities) without requiring any modifications to the end-hosts}}. Given that most rural users are not highly mobile, VC-ISP identity management supports limited mobility within a set of neighboring VCNs in a graceful manner but is not designed to support super high mobility users. This layer also allow users and services to discover other entities within the network using their conventional names. We note that the identity management layer of VC-ISP replaces many of the conventional lookup and resolution protocols used in conventional 3G and 4G cellular networks.\textcolor{red}{Talal: We can not connect just wifi  devices to our network and not with their names, we can only connect GSM devices. Without a sim card, even the GSM device won't connect. So I don't think we can claim that we allow all wifi devices to connect. We should pitch this as a parallel software based naming addressing instead of a hardware based naming addressing, we have to say that this naming and addressing is fundamentally different from the way identities are in conventional network. We have to argue why this is more faster, fault tolerant, distributed and not dependent on proprietary hardware compared with conventional cellular design. Follow up question again is: is this going to be fundamental enough a contribution to get this paper in. } 

{\em 4. Distributed Mobile Edge Services:} Given the edge programmability, VC-ISP provides new application primitives to enable new forms of \st{intermittency-aware}, cloud-controlled, distributed, mobile edge services where every VCN maintains critical application state to enable mobile services to function in an intermittency aware manner in the face of unreliable backhauls and network failures. These services are also {\em distributed} in the sense that users across VCNs can cooperate and run different types of peer-peer applications and community-specific applications. We demonstrate a spectrum of applications that we have built on top of the VC-ISP primitives including P2P transactions, voice-based social media applications, P2P messaging and distributed mobile sensing applications. \textcolor{red}{Talal: What eval should we have for intermittency awareness? And more importantly, what do we claim when we say intermittency-aware applications? Is it the same as in case of failures we perform better... in that case the VCF, CCF eval we have should be enough for this. Although it is all simulation based. I need some clarity on this. I mean above is the only thing that comes to my mind with respect to intermittency awareness }

We demonstrate the effectiveness of the VC-ISP model using a real-world 3-node VC-ISP deployment including a solar-powered cell tower installation in rural Ghana. Our Ghana installation also supports different types of distributed mobile services (as outlined earlier) that have been used by rural users within the community. In addition, we evaluate the effectiveness of specific aspects of the VC-ISP architecture using emulation and simulation experiments. In summary, we believe that VC-ISP represents a radical departure from the conventional thinking of how we design cellular networks and could enable ground-up innovation where several budding rural entrepreneurs could launch competing cellular network services in rural localities while seamlessly co-existing with existing operators.



%The goal of having low latency is central in various networking services and is even more important in context of rural areas because of low bandwidth. While some applications like real time applications inherently require low latency to work, other services like web content delivery and VoIP aim to reduce latency to improve customer satisfaction. The distance of resources from clients is the key reason for latency apart from link bandwidth. Content replication and caching is often seen as a solution web infrastructure but the hardware and software resources are primarily focused in developed regions and high latency is experienced by people of developing countries because of being far away.

%In comparison conventional cellular networks are inflexible because of their brittle architecture. To route traffic and perform fine-grained packet processing, conventional cellular providers rely on specialized and proprietary devices, namely: Serving Gateways (S-GWs) and Packet data network Gateways (P-GWs). S-GWs are mainly used as mobility anchors to provide seamless mobility. P-GWs centralize most network functions like content filtering, traffic optimization, firewalls, and lawful intercept. P-GWs sit at the boundary of the cellular network and the Internet. The base stations, S-GWs, and P-GWs communicate using GPRS Tunneling Protocol (GTP). Centralizing nearly all data-plane functionalities in the P-GWs makes cellular core networks remarkably inefficient, complex, and inflexible. Even the device-to-device traffic and local content distribution network services are handled by P-GWs. This increases the network delay and congestion. The P-GWs are not modular, carriers often end up paying for functionalities they do not need; when a function is not available, carriers have no choice but to replace the P-GWs. Contradictory to this we connect each of our node to the internet directly and each node and have much more software flexibility for making routing decisions at the bts node. 
%These are not the only problems that are faced by developing countries. Energy infrastructure is another major challenge which translates to millions of people living without connectivity. Due to total or intermittent lack of grid power in vast areas of developing regions and high power consumption of cellular base stations and backhauls, it becomes extremely difficult to run cellular networks in an economically viable manner beyond a certain point. Laying new infrastructure is a considerable cost and if the profit returns are not substantial, commercial cellular networks have no incentive to provide any connectivity. 
%Backhauls are an important part of any networking service that wants to operate in rural areas. While there are options like satellite and long range wifi, they are either very expensive or require a significant engineering effort along with line of sight between connecting points. There is a need to build an alternative backhaul by using the weak cellular signal at the edge of cellular coverage because sporadic cellular coverage is often available in a lot of remote areas. We use signal boosters and link aggregation to build a relatively high bandwidth backhaul available in the area. As the rest of the components of our platform the backhaul is also low-cost and has a low-energy profile.

%There is a need of a unifying architecture for providing a \textit{virtual} cellular ISP abstraction that can help connect different VCNs in a seamless and scalable manner. The VC-ISP will enable multiple community based VCNs to connect to each other and provide an array of useful services that a real cellular network can provide while dealing with the challenges of low bandwidth delay ratio(low BDR) backhauls and operating in licensed GSM spectrum.  %A good solution is not only cheap, convenient and easy to use but is one which is also scalable and provides a better management interface for larger, distributed deployments whilst ensuring QoS requirements for all connected communities.

%We show that this is a low-cost, low-power fully customizable solution that can be used to bring cellular coverage to areas that don't have coverage and provide various services with low latency and high quality as compared to a regular base station. The rest of the paper is organized as follows. In section 2 we explain the problem context and motivation for this work. In section 3 we give the system architecture. In section 4 we give the details of programmable platform. In section 5 we give the details of the services we supported in our platform. In Section 6 we give the implementation and deployment details. In section 7 we give the evaluation. In section 8 we give related works and section 9 is conclusion. 

 


==> content/2-context.tex <==
\section{Motivation}
\label{sec:motiv}
\textcolor{red}{Talal: This text probably needs to go away because we need the space we are wasting on this and intro is covering this stuff. We can probably move the useful figures above if we want}

In this section, we try to explain the plethora of problems faced by developing countries when it comes to connectivity. We focus on 4 problems in particular which motivate our design decisions.

\subsection{Latency And Bandwidth}

Web access in developing countries is slower when compared to the rest of the world \cite{akamai}. One would believe that these issues persist due to the growing disparity between infrastructural support and page complexities where the latter far outgrows the former \cite{klotski}. However, Accra the capital city of Ghana which is well connected by undersea cables~\cite{cable} continues to experience high latency~\cite{yasir_imc}, suggesting the problem lies elsewhere. A recent study \cite{yasir_imc} shows that for various traces from different locations in Ghana, DNS lookup is one of the major factors (nearly 37-47\% ) for high user-perceived latency. Similar findings have been made by other studies in developing countries \cite{koradia2013first,chetty2013measuring}. This high DNS lookup time has been attributed to the uneven distribution of DNS name servers around the world. This highlights the fact that the location (and quality) of resources and services can have a huge impact on user perceived latency. 

\subsection{Cellular Coverage}

As mentioned earlier in \S 1, an estimated 1 billion people live without cellular coverage worldwide. This lack of coverage is primarily due to low population densities in these areas which translates to lower profit margins for commercial providers. Data indicates that the cellular coverage of regions in Panama directly correlate to its population density. %Similar is true for other developing countries. 
This absence of cellular connectivity plagues regions with further economic recession \cite{jensen2007digital,aker2010mobile}.

%\begin{figure}
%  \centering
%  \includegraphics[scale=0.3]{figures/coveragemap_panama}
%  \includegraphics[scale=0.25]{figures/popmap_panama}
%  \caption{Top is the cellular coverage map of Panama and bottom is the population density map of Panama.\label{fig:panama}}
%\end{figure}

\subsection{Application Diversity \& Support}

In recent years, deployment of small scale community based VCNs \cite{kurtis_ictd,anand,zheleva,rhizo} have come to prominence. These deployments stemmed from the growth of interest around new software \cite{openbts} and hardware \cite{range,endaga}. Though they assuage the connectivity issues, they only focus on providing the very basic cellular functionality. Additionally, Internet access in most of the rural areas is mostly through mobile phones connected to conventional networks. Studies have shown that people are cautious of data usage because of the cost associated with it \cite{blah}. Naturally, mobile applications that are both cost-efficient and beneficial to the daily needs of the inhabitants are more preferred \cite{dalvitdata}. Thus, the needs of such community members are twofold: (a) reduced bandwidth consumption and (b) the need for useful, relevant applications. 

For routing and fine-grained packet processing, conventional cellular providers rely on specialized and proprietary devices for extensive processing at the core. This also implies that they don't have a chance to choose between different capabilities from different providers to mix and match hardware~\cite{chiosi2012network,jin2013softcell}. Thus, the brittle architecture of commercial cellular networks adds several overheads which come at high financial and temporal costs. To elaborate, if a community wants a small sensor application to collect mapping data related to farms, the application server has to be deployed within a data center inside the cellular network or somewhere in the cloud. This will additionally increase the latency (temporal costs) and create a routing overhead between the small community to the server. More often than not, this mammoth infrastructure (and associated financial costs) is not required to service such trivial applications.

\subsection{Power Infrastructure}

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|}
\hline
Grid Power not available (hrs) & Percentage of sites \\ \hline
$0 < x < 2$ & 11.2\% \\
$2\leq x < 5$ & 22.0\% \\
$5 \leq x < 10$ & 48.0\% \\
$x\geq 10$ & 18.8\% \\ \hline
\end{tabular}
\end{center}
\caption{The distribution of power outage across sites. $x$ denotes the number of hours grid electricity was not available.}

\label{tab:poweroutages}
\end{table}

The 2014 Africa energy outlook report states that 620 million people live without electricity in sub-Saharan Africa \cite{outlook}. This leads to unrest among conventional cellular network providers who have to additionally invest to provide the required power infrastructure for even trivial operation. A single GSM base station could consume anywhere between $5-10$ kW in urban areas with lower power levels and $10-20$ kW with higher power levels \cite{basestationpower}. Even when available, the grid electricity is highly unstable. According to a cellular provider in South India, the voltage can fluctuate between -1000 V and +1000 V causing device failures \cite{blah}. Table~\ref{tab:poweroutages} reflects the power availability based on data obtained from a cellular provider in South Asia. This data is from over $1000$ sites within a region for a single day in $2014$. The first column in the table is the duration of grid failure and the second column is the percentage of sites that faced it. It is worth noting that nearly $19$\% of the sites faced over $10$ hours of grid failure related issues. To compound issues, these failures can sometimes last across days. This leads to a heavy dependence on Diesel powered generators to provide {\em reliable} cellular services in developing countries \cite{ahmad2015solar}. 

\subsection{Usable Spectrum}

All wireless communication signals travel over the air via radio frequency (or spectrum). Government agencies such as the Federal Communications Commission (FCC) license (or allocate for usage) specific slivers of the available spectrum to conventional carriers. GSM Whitespaces are defined as the licensed spectrum that is unused in a particular geographic area by these conventional carriers \cite{gsmws}. Though licensing happens at a fine-grained level, whitespaces are common as the entire chunk of allocated spectrum is not required for providing the required functionality. Thus, any under served area is guaranteed to have an excess of unused spectrum in all GSM bands. 





==> content/3-arch-new.tex <==
\section{VC-ISP Architecture}

\begin{figure}
\centering
{
	\includegraphics[scale=0.4]{figures/SystemArchitecture6.pdf}
}
\caption{VC-ISP Architecture}
\label{fig:systemArch}
\end{figure}

The VC-ISP is a new model for designing and rethinking the evolution of cellular network providers. The network architecture comprises of a distributed collection of software-defined VCNs powered by emerging open-source cellular base-station platforms that together provide the abstraction of a single virtual network with the entire gamut of features offered by a traditional cellular provider. Using this architecture, we wish to extend coverage beyond existing boundaries, moving a wide variety of services to the extreme edge. The VC-ISP network architecture aims to enable third-party vendors to offer cellular ISP services in a decentralized manner without making any modifications to mobile devices and in cooperation with traditional cellular networks.

{\S \ref{sec:motiv} discusses several motivational factors that influenced the design of the VC-ISP architecture. These factors are relevant to the architecture as it is directly inspired by VCNs. We refer to a single VCN in a VC-ISP as a {\em node} - a programmable, software-defined, local cellular network which can provide the basic suite of cellular services ranging from voice, data and messaging capabilities to connected clients. Conventional cellular networks continue to use highly inflexible and expensive platforms with complex control-plane protocols making the network nearly impossible to configure or manage. On the contrary, programmable platforms such as OpenBTS \cite{openbts} enable us to program and easily integrate a wide range of other middlebox services and functionalities. The strawman architecture is illustrated in Figure~\ref{fig:systemArch}; a distribution of nodes provide access to a geographically disjoint set of regions and collectively provide the abstraction of an unified VC-ISP. We envision all the nodes to be connected to the Internet using various types of backhaul technologies such as wireless backhauls, satellite links, balloons \cite{loon}, leased lines, telephony, fiber etc. Owned by a single party, a centralized cloud controller interconnects all nodes and is in charge of administering this cohesive network. This controller resides at an appropriately placed geographic location to normalize communication latency. To achieve such an architecture, we discuss design specifications and the high level goals we wish to achieve. To summarize, the architecture should be able to:

\begin{itemize}
\itemsep-0.23em
\item {\em Goal 1:} Operate in regions where there is high latency, low bandwidth and intermittency.
\item {\em Goal 2:} Operate in regions where conventional cellular is inaccessible or sparsely available.
\item {\em Goal 3:} Reduce processing at the core and migrate relevant application processing to the edge to further reduce latency.
\item {\em Goal 4:} Avoid placing heavy reliance on conventional sources of power (including fossil fuels). 
\end{itemize}

Addressing these goals would require us to tackle several research challenges. The first and foremost challenge involves the exploration of a variety of operational conditions. These introduce research challenges both for handling competition and cooperation between providers. Cellular spectrum is a resource under contention and VC-ISP needs to operate in white spaces not overlapping with the spectrum of traditional providers. 

Additionally, majority of developing regions have poor cloud infrastructure and a weak backhaul, resulting in low Bandwidth-Delay Ratio (BDR) regimes. Traditionally designed applications running in these regimes face several issues including frequent timeouts, operational bandwidth insufficiency and various other inconsistencies. Dealing with these issues and obtaining {\em Goal 1} requires rethinking application requirements. Mobile clients are henceforth connected to a {\em local} server placed in the proximity of the base station. This local server has complete autonomy in making decisions for a certain class of events but also abide to directives from the central controller. Therefore, the local server ensures greater responsiveness to the clients. Inconsistencies are avoided by relaxing the consistency guarantees and providing lazy synchronization with the cloud. The VC-ISP will provide a separate intermittency-aware substrate where all messages are tagged with session and communication group specific identifiers that enable nodes to store and deliver messages to the corresponding recipients in a delay-tolerant manner; mobile applications in VC-ISP can also leverage this substrate to specify how to handle application specific messages in an intermittency condition. 

Every node in the VC-ISP runs the OpenBTS platform which offers a software-defined cellular abstraction. Being equipped with a software-PBX allows the node to continue offering basic communication services despite the weak backhaul. This is not possible in conventional cellular networks which require multiple components (often located at different locations) to enable a call between users connected to the same base station. However, to improve performance, operate in the extension of existing coverage, and to obtain {\em Goal 2}, we are required to amplify the available signal. Aggregated bandwidth is achieved through the use of directional antennae and parallel boosted links. 

A centralized cloud infrastructure provides mechanisms for the now unified (nodal) network to communicate with the non-member networks. This infrastructure comprises of has 2 key components:

\begin{itemize}
\itemsep-0.23em
\item {\em Egress nodes}, which are responsible for forwarding traffic either between VCNs or between VCNs and the conventional cellular network. 
\item {\em Lookup and messaging servers}, which play a critical role in enabling the VC-ISP to offer connectivity and a variety of cellular services across nodes. 
\end{itemize}

Each node in the network operates independently and communicates with other VCNs using the egress nodes, and the lookup and messaging servers. We partially obtain {\em Goal 3} as the local servers help facilitate this process in most cases because they have a cached version of the naming and addressing table. As these servers also have administrative autonomy, they are able to act on the behest of the centralized controller providing additional services for applications at the extreme edge. Different types of edge services will be explained in subsequent sections.

The modular nature of the various components required to build the VC-ISP ensures minimal power consumption. Therefore, we obtain {\em Goal 4} by predominantly powering the nodes using solar panels. By building a compact, mobile base station unit, we are able to the reliance on the unstable grid power in these regions. 


==> content/4-archspecs.tex <==
\section{VCN building block}
\label{sec:opp}



%Most content in this section and sections to follow are based on information obtained from our VC-ISP deployment comprising of 3 VCNs; one each in Kumawu, Abu Dhabi and New York. We believe that the insights and results obtained from this deployment will scale with the number of VCNs and VC-ISPs and show specific evaluation to support our claim in \S \ref{}. Subsequent subsections elaborate the white spaces detection, boosting backhauls and failure handling in our architecture.
\textcolor{red}{
Talal: Rewrite white spaces. Only focus on our solution. And then we need to say why it is different from just a participatory sensory framework adding the database detailed algorithm and how competing VC-ISPs collaborate/compete in the same area will provide coverage. In reliable back haul talk about the sigcomm demo in a little more detail. If the key contribution is that we can aggregate multiple parallel links Operating in areas where there is no signal we have to show aggregation. I don't know how to do that at this point and what is feasable in Ghana. Designed for extended backhaul. One is a boosted backhaul and the other is just a wireless link. When it comes to backhaul. 4.3 in my view is useless and needs to go. }

The two most basic building blocks required for any VCN are a back haul and a mechanism to operate without interfering with the incumbent providers. 


\subsection{Detecting White Spaces}	
\label{sec:gsm}

Wireless spectrum is auctioned on a regular basis to telecommunication organizations. Though licensed in its entirety, majority of these slivers remain unused in developing regions. The existence of these unused bands of spectrum, collectively called GSM white spaces, has been proved for a remote area in Indonesia, and a system has been built to operate without interfering with the licensed providers \cite{gsmws}. Proposed by Hassan et al., Nomadic GSM (NGSM) \cite{gsmws} safely uses unused licensed spectrum without requiring cooperation or participation from existing license holders. NGSM takes advantage of the fact that GSM handsets continually measure spectrum occupancy in their proximity and report these measurements to their serving cell to aggregate, ergo mitigating the practical impact of the hidden node problem caused by client side interference. However, NGSM has the following limitations:

\begin{enumerate}
\itemsep-0.23em

\item The design necessitates two base stations in the same location, so that active calls in the primary can be moved to the secondary when the primary is collapsed. 

\item The secondary base station begins to transmit at full power on a randomly chosen Absolute Radio Frequency channel Number (ARFCN) even before any sensing is done. This can lead to interference with a primary operating in that ARFCN. 

\item Often, the status quo in developing regions is the reduced frequency in call or SMS between users. This results in the measurement reports to the serving cell become infrequent. A major consequence is delayed readings, which can further lead to wrongfully using a channel that interferes with a primary license holder. 

\end{enumerate}

To alleviate the above limitations, we created a GSM white spaces detection mechanism similar to NGSM. We use is a hybrid of participatory sensing and database approaches where mobile devices measure spectrum occupancy over a larger area in a distributed manner, and share these reports with the serving cell to aggregate. We remediate NGSM's first limitation by not necessitating the presence of two different base stations. Instead, we wait for the connected calls to complete in case it is time to shift to a different channel. Though weaker, this solution is more pragmatic and economically feasible. The second limitation is mitigated by increasing transmission power periodically to slowly expand coverage. This is done while simultaneously sensing for used channels among a list of safe channels. Thus, a small software-defined base station can be installed at any location without examining the spectrum prior, because any interference caused will be at a much smaller radius than compared to a base station transmitting at full power. The final limitation is addressed using a custom mobile application that periodically makes calls and sends messages to the base station. This ensures periodicity, ergo frequency in measurement reports. If a few volunteers in the community run this application, the cost associated with additional calls and messages can be divided across all community members to ensure only a nominal increase in their payments. 

\subsection{Reliable Backhauls}
\label{sec:backhaul}

In a hierarchical telecommunications network, the backhaul comprises of the intermediate links between the core network and smaller subnetworks. Cell phones communicating with a single base station constitute a local subnetwork; the connection between the cell tower and the rest of the world begins with a backhaul link to the core of the ISP's network. However, a significant percentage of cellular users suffer from poor signal strength due to a weakened backhaul and the problem is exacerbated in peri-urban areas in developing regions. In the VC-ISP architecture, our focus in on end-users in such small localities who can benefit from increased bandwidth cellular connectivity, especially when the area receives relatively poor cellular signal strength. We devise a strategy such that with minimal effort, one can build effective directional cellular backhauls by aggregating independent cellular connections amplified using signal boosters. 

Our solution for signal amplification is orthogonal to the design of various Line of Sight (LOS) and Non Line of Sight Cellular (NLOS) backhauls \cite{tarana,kumu,wildnet}. It involves the usage of a directional cellular backhaul comprising of a directional outdoor antenna, signal booster, and an indoor antenna to provide the amplified signal within a highly constrained area. Specifications for the directional antenna include a set up height of at least 10 feet above the repeater and indoor antenna to minimize interference. The indoor setup aggregates multiple, independent cellular connections powered by their own SIM into a single boosted backhaul. For the results reported in \S \ref{}, we used an zBoost CANT-0042 outdoor directional antenna, connected to a signal booster to a 30-foot long coaxial cable connecting to an indoor antenna. To effectively combine multiple cellular connections into a single directional backhaul link, we use Ubuntu Bonding module \cite{bonding} which provides a method for aggregating multiple Network Interface Controllers (NICs) into a single logical bonded interface of two or more NIC slaves. We discuss the efficacy of this approach in \S \ref{}. 


\subsection{Fault Tolerance}
\label{subsec:ft}

Coupled with standard failure scenarios that arise due to the distributed nature of the architecture, failures can exist due to the extreme operational environments. Unlike standard distributed systems where the network is not considered the bottleneck, our network is often unreliable, has high latency and limited bandwidth, and often heterogeneous. Added to the standard failures of hardware and software, these network uncertainties can result in failures of (a) links between the nodes and the cloud, and (b) either local servers, cloud servers, or both. Though unimplemented, we believe that commonly used solutions such as heartbeating \cite{hayashibara2002failure} can be used to check for partitions, whilst weaker forms of consistency provide a fix during reconciliation for the first failure scenario. A suitable transport layer protocol with an adequate TTL period is required in the deliberation of availability against reliability. In case of the second scenario, typically used solutions involve content replication of the local/cloud server to a secondary, the use of a replicated state machine, a Paxos group or any distributed consensus protocol. Naive approaches involving a dedicated log server are not popular as extensive monitoring can cause delays, occupy additional space and potentially interfere with normal operations.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                

% {\bf Link Failures:} Broadly speaking, the links between the nodes and the cloud controller are crucial given the low-BDR, high intermittency environments, both for providing VCN facilities comprising primarily of communication related tasks and for providing support to various applications that are required to operate in these harsh environments. In the event of such a failure, local servers at a nodal level have some degree of administrative autonomy and can provide moderate support for applications at the extreme edge. This involves buffering requests that cannot be serviced whilst resolving others. Though new identities can not be generated for clients joining the nodes during such partitioning, these requests are also queued in order and serviced accordingly once the link is up. By providing services at the extreme edge, we are able to reduce the frequency of communication with the central controller for certain high priority tasks and increase availability in the time of partitioning, at the expense of stronger consistency guarantees \cite{attiya1994sequential}. Commonly used solutions such as heartbeating \cite{hayashibara2002failure} can be used to check for partitions, whilst weaker forms of consistency provide a fix during reconciliation. A suitable transport layer protocol with an adequate TTL period is required in the deliberation of availability against reliability.
% 
% {\bf Node/Cloud Failures:} A more serious failure involves that of the local server at the nodal level, or failure of the cloud controller. As the local server facilitates edge services, its absence hinders the progress of multiple applications for all clients connected to that node. Applications that can circumvent the local server still work during such failures at the expense of longer communication periods. Applications that can function assisted by the local server continue to persist in the event of a cloud failure at the expense of extensive local logging. Though not implemented, typically used solutions to deal with such form of failures involve content replication of the local/cloud server to a secondary, the use of a replicated state machine, a Paxos group or any distributed consensus protocol. Naive approaches involving a dedicated log server are not popular as extensive monitoring can cause delays, occupy additional space and potentially interfere with normal operations.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                


==> content/5-idmanagement.tex <==
\section{Naming \& Addressing}
\label{sec:idmanage}

%\begin{figure}
%\centering
%        \includegraphics[scale=0.25]{dht.pdf}
%\caption{Architecture picture for a more scalable \name architecture with multiple nodes connected to multiple cloud controllers that form a DHT based mechanism for storage and satisfying other requests}
%\label{dht}
%\end{figure}

\textcolor{red}{Talal: There is a need for subsection before 5.1 that highlights why do we even need a new identity management framework. This section should go into details of how identities are handled in conventional cellular networks and how mobility and handovers are handled. Then we need to go into our solution and how we provide flexibility and uniqueness and mobility across the VCNs close by and when users go to a different VCN and why do we make the choices that we make and how it is better. This has to lay some groundwork for the VCE and GCE error graphs that we create. }

To successfully utilize the various services of cellular networks, even from outside the network, it is imperative to have an efficient scheme for device naming and addressing. We wish to achieve three goals using our identity management service, namely (a) flexibility in identities held, (b) seamless user experience, and (c) uniqueness. 


\subsection{Flexibility}
\label{subsec:flex}

A user can have an identity which authenticates her to use applications offered by the \name. However, this identity should not facilitate communication with external users (outside the VC-ISP). Similarly, a user can have another identity whose sole purpose is to enable communication with the outside world. To this end, the VC-ISP issues two types of identities: {\em (a) Local identities} that are only usable/valid inside the VC-ISP framework, and {\em (b) Global identities} which make it possible for devices outside the framework to connect with those inside. It is the duty of the identity management service to multiplex the functionalities accordingly based on the nature of the identity. 

Apart from being enabled to utilize application support within the VC-ISP, users with local identities can communicate with others within the same VCN or in the same \name. In contrast, global identities provide all the functionalities supported by local identities and enable connection both to and from outside the \name. The importance of this form of flexibility stems from the fact that providing access to an identity outside the network has an associated cost. Globally identifiable names need to be purchased (or leased on a monthly basis) from organizations selling VoIP services, like Nexmo \cite{nexmo}. Users must be given a choice to be reachable by those outside as they are required to bear the cost associated with the leasing or subsequent purchase of the corresponding identifier. This flexibility in choice is currently unavailable in any conventional cellular network. 

\subsubsection{Generation \& Dissemination}
\label{subsubsec:gnd}

Unique identifiers are maintained, regulated and generated (sequentially, in the order in which requests are received) by a centralized server different from the controller, henceforth referred to as a name server. These identifiers (or names) are flat and carry no location information. The flexibility offered in naming can best be utilized when the architecture is optimally designed. To achieve the required performance, we have two different implementations, namely:

{\bf 1. Server-Client Model:} A single, centralized name server issues both global and local identities as requested. If a new users enter any node, the registration requests are routed to this name server in the order of entrance. In the case of a cellular device that connects through the OpenBTS interface, the request to generate a name comprises of the IMSI number (which is globally unique and non-mutable). This information is then used in the standard GSM challenge-response protocol, when the phone associates with the network. The response from the central name server is a unique identifier. This server keeps track of each identity issued (name) and its current location (address), maintaining consistent state information. This information is required to route calls and messages correctly. In addition, it records the IMSI number of the SIM card to which the identity was issued. If the user moves to a different node, the server still knows that an identity has been issued and only the location of the user needs to be updated. To reduce communication latency, this information is replicated at the local servers at a nodal level and updated on occurrence of a cache-miss. It is easy to envision a hierarchical model where a centralized name server branches into several sub-name servers which are independently responsible for naming and addressing disjoint nodes. However, this approach does not scale if the distribution of users is uneven among the nodes.

{\bf 2. DHT-based Model:} Nodes obtain an identity from a centralized name server as discussed in the previous approach. However, all other functionality required by the node are provided by a cloud controller chosen based on a predefined hash function. These cloud controllers are located in data centers nearest to them ensuring the presence of high bandwidth links between each other. Combined with a central name server, these cloud controllers collectively form a DHT for managing identities and application level data storage. This DHT-based model used by several authors \cite{wire,seattle} deals with failures and provides faster access even when there is a skew in users between different nodes by evenly dividing storage and processing. 

{\em Intermittency aware lookup:} As explained earlier, the VC-ISP architecture provides an eventually consistent view of the entire name space to the local server at a nodal level. If a client requires information of another, it first contacts the local server of the node it currently is in. On occurrence of a cache-miss at this node, the required information is retrieved using suitable cache-update protocols \cite{puzak1985analysis} in a lazy manner. In the absence of a backhaul to the central name server, information at the local server at the nodal level is zonally consistent. As with the name server hierarchy, we define a {\em zone} to be a set of smaller nodes that are downstream a larger node, including the larger node. This suggests the existence of a functional communication link between the larger node and all its downstream peers despite the intermittence, a feature possible because of support provided by OpenBTS and the geographic proximity of various nodes in the zone. One can imagine a zone to comprise of smaller villages where each village has a node of its own.

\subsection{Seamless User Experience}
\label{subsec:seamless}

In both of the above discussed models, naming and addressing information is cached at the local servers at each node. Though not complete, caching ensures a reduction in communication latency in the case of lookups, ergo improving the end-user experience. 

{\em Interoperability:} It is crucial for the architecture to support the following: (a) communication within the VC-ISP, (b) communication across VC-ISPs, and (c) communication between VC-ISP and non-member networks (in both directions). Communication with the architecture is explained in previous sections, where information obtain from the combination cache hits and misses on local servers and the centralized name server suffice to locate a given identity and ensue communication. Communication across VC-ISPs necessitate a federation manager, an entity responsible for aggregating both name and addressing information across all VC-ISPs. At the expense of a lookup to this manager, members of a particular VC-ISP can locate those at another VC-ISP. In our current hierarchy, the federation manager is at a level above the cloud controller and central name server so as to provide it a better view of the organization below. To better understand the third case, consider a scenario where a client with a global identity wishes to contact someone outside the node who is not part of the VC-ISP i.e a contact in a non-member network. On entering the contact's information, the identity management system in the local server generates a cache miss. A subsequent check at the central name server also results in a miss as the contact's naming and addressing information belongs to a third party telecommunication organization. On observing both misses, the local server redirects the communication request to the cloud server, which further forwards this request to the VoIP service provider from whom the global identity was purchased. It is now the responsibility of the service provider to appropriately route the communication request. Thus, any client with a global identity can communicate with a contact outside the VC-ISP architecture without entering any additional information and vice-versa. It is important to note that clients with local identities can effectively communicate with other clients within the VC-ISP using a similar mechanism of cache and central name server lookup to locate the address of an identity. The key difference is that the calls are routed within the VC-ISP architecture using OpenBTS and not a VoIP service provider.

{\em Mobility:} The entire VC-ISP architecture is designed to extend coverage at the existing boundaries; we do not anticipate mobility in great frequency and displacement. Thus, the zonally consistent view of the name (and addressing) space and facilitates moderate mobility within the zone without the expense of dropped communication. However, larger amounts of displacement coupled with lazy synchronization (eventual consistency) require communication buffer at a nodal level to ensure correctness.

\subsection{Uniqueness}
\label{subsec:unique}

Though local servers at the nodal level have some degree of administrative autonomy, only the centralized name server issues identities to all nodal clients to avoid naming conflicts. The central name server produces identities sequentially in the order at which it receives the requests. Though the generation of an identity comes at the expense of an additional hop to the central name server, this cost is amortized as the information is eventually replicated and cached in the local server at the nodal level, subsequently minimizing communication latency as well. Standard cache population algorithms are used to ensure the freshness and efficiency of the local cache. This uniqueness in naming is essential to ensure calls and messages are routed to the correct destination.








==> content/6-applications.tex <==
\section{Applications}
\label{sec:app}
\textcolor{red}{Talal: I am largely satisfied with this section's contents. The only problem for me is that it has not been properly motivated. We need to probably motivate for it a little bit. To me this section needs to be articulated as an advantage we get for choosing VC-ISP architecture over conventional cellular. Also to answer the question how does a VC-ISP work for applications. } 

In this section, we highlight the application primitives we built that enable distributed and highly available applications atop the \name. However, supporting such applications in a conventional cellular network requires deployment of application level code after the packet gateways (P-Gateways). This is intractable as the latency between a mobile phone and packet gateway can be 100 ms or more. In our architecture, each application leverages the software processing capability at the extreme edge (local servers), consequently dividing it into a local component and cloud component. With the help of our application primitives layer and packet routing ability at the base station we are able to deploy applications very close to the users. We encapsulate network management in application level primitives to help facilitate intermittency awareness. This can help reduce the latency and better manage the backhaul. 

\subsection{Primitives}
\label{subsec:prim}

The main focus of primitives is to enable the applications to choose between consistency and availability. Since most VCNs are located in low-BDR regions we achieve partial availability by dividing each application into a larger local component and a smaller cloud component. The local component of the application ensures that significant processing is achieved locally. This ensures partial application responsiveness by keeping local communication and interaction functional even in the absence of the low-BDR backhaul link (\S \ref{subsec:ft}). The cloud component is mainly responsible for saving application data and facilitating interaction amidst local components across VCNs. The lack of programmability in conventional cellular networks forces application deployment extensively in the cloud. This means that failure of a backhaul link between the base station and cloud inhibits access to even basic applications like calls and SMS. These primitives we designed hide the internal implementation of the components discussed in \S \ref{sec:opp}, and include:

\noindent{\texttt{1. SLOWPUT(Identity i, Type t, Data d)}}: 

\noindent{This primitive is used by the local component for {\em lazy} communication with the cloud component. Particulars include a user \texttt{i} communicating marshalled data \texttt{d} for application \texttt{t}. This operation is lazy because data may not be immediately sent after the primitive is executed; the local server determines the right order to send the data based on bandwidth availability and priority (based on \texttt{t}) of the other requests in the queue. The \texttt{SLOWPUT} primitive is used by applications for which the local component can provide availability at the expense of strong consistency. For example if someone is just try to send an e-mail from VCN $A$ to a user connected to VCN $B$, any inconsistency in the ordering of e-mails at receiver is tolerable.}

\noindent{\texttt{2. FASTGET(Identity i, Type t, Data d)}}: 

\noindent{This primitive is used by the local component of any application to send and receive data from the cloud component in an {\em active} manner. The particulars include a user \texttt{i} communicating data \texttt{d} for application \texttt{t}. This primitive is usually called as a result of an application function when consistency and response time can not be compromised. The communication is not queued, as in \texttt{SLOWPUT} primitive. Instead, this primitive is executed instantaneously, provided the the backhaul link is active. For example, any inconsistencies in the case of a banking transaction are grave, and an interactive response is required almost immediately. Such applications require the \texttt{FASTGET} primitive and marshall the transaction in the data parameter, forwarding it to the central component of the banking application.}

\noindent{\texttt{3. FASTSEARCH(Identity i, Type t, Data d)}}: 

\noindent{This primitive is used by the user \texttt{i} to search for data \texttt{d} of a particular application type \texttt{t}, and returns one or more data points based on search from the cloud component's data store. The communication encapsulated by the \texttt{FASTSEARCH} primitive occurs instantaneously. The \texttt{FASTSEARCH} primitive executes a read operation on the persistent storage of the cloud component, therefore it can be performed even if a \texttt{FASTGET} operation has a write lock. An example use-case of the \texttt{FASTSEARCH} primitive can be to search in the data store of cloud component while a user is on hold with an IVR-based application, and is expecting a response on a read query.} 

\subsection{Examples}
\label{subsec:example}

In this subsection, we give the examples of applications that we built for developing regions using the primitives discussed above. In particular, we highlight how a functional division is made to identify the functions that require consistency to those that require availability. 

\subsubsection{P2P Transactions}

The application provides a text-based interface (running on top of the SMS service) and enables traders to provide customers the price and quantity of a commodity (usually crops) they wish to sell. It also enables customers to search for a particular commodity, the price at which various traders are selling, and to place a \texttt{BUY} request. The \texttt{BUY} request leads to exchange of contact information between transacting parties, and is logged as a \texttt{SELL}. The text-based interface requires small phrases to commence transactions.

The heart of the application's local component is the \texttt{ReceiveHandler}, which uses the above defined primitives to communicate with the cloud component. The lazy \texttt{SLOWPUT} is used send the data to the server, on sale of a commodity. In case the user is interested in purchasing a commodity, \texttt{FASTSEARCH} is used, and the data returned is sent to the user over one or more text messages.Relevant data is marshalled by the local component into the \texttt{info} variable. The cloud component is responsible for any subsequent unmarshalling. 

%\begin{algorithm}
%\caption{Local server algorithm}
%\label{CHalgorithm}
%\begin{algorithmic}
%\Procedure{Marketplace\textendash Receive Handler}{}
%\State $...$
%\If{Seller}
%\State SLOWPUT(user,Marketplace,info)
%\ElsIf{Buyer and Searching}
%\State FASTSEARCH(user,Marketplace,info)
%\ElsIf{Buyer and Buying}
%\State FASTGET(user,Marketplace,info)
%\EndIf
%\State $...$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

\subsubsection{IVR-Based Social Media}

This application enables users to interact with the system by pressing numbers on the phone's keypad. It enables users to leave a message, or to listen to a message left by others. For the Ghana VCN, the application provided an option to either use English or Twi, the local language in the region. The key function is thel \texttt{ReceiveHandler} at the local component, which is invoked using a HTTP request on entering the IVR extension. After the initial HTTP request, the call is bridged from base station to the Asterisk IVR server running as the local component of application. The Asterisk server logs each input of user as entered. If the user is recording a message, the \texttt{ReceiveHandler} is executed after its completion. The \texttt{ReceiveHandler} uses the lazy \texttt{SLOWPUT} primitive to send the recorded file to the cloud component. In case a person wants to listen to a message, the function first checks if the validity of the session. If the session is valid the message is played locally. Otherwise \texttt{FASTSEARCH}  and \texttt{FASTGET} primitives are used to search and fetch the most recent message from the cloud component, while the user is on hold.
%
%\begin{algorithm}
%\caption{Local server algorithm for IVR}
%\label{ivr_algo}
%\begin{algorithmic}
%\Procedure{IVR\textendash Receive Handler}{}
%\State $...$
%\If{Recorder}
%\State $localProcessing()$
%\State $SLOWPUT(user,SocialMedia,message)$
%\ElsIf{Listener AND SesssionValid}
%\State $playLocal()$
%\Else
%\State $FASTSEARCH(user,SocialMedia,messageType)$
%\State $FASTGET(user,SocialMedia, messageId)$
%\State $playLocal()$
%\EndIf
%\State $...$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}


\subsubsection{Distributed Data Gathering \& Sensing}

The purpose of the application was to collect data on farms and crops grown. The application provides an interface to create the map of any farm by walking along its edge. This data is sent to the local application component, an HTTP server next to the base station. The local component then uses \texttt{SLOWPUT} to upload this data to the cloud component. Our choice in primitive is valid as the application does not require strong consistency and we can afford to have unordered data at the cloud component. This application is relatively simple because data only needs to be uploaded to the cloud component of the application, and there is no need for downloading data.

 


==> content/7-a_impl.tex <==
\section{Implementation}
\label{sec:implementation}

In this section, we describe in greater detail how we implement different parts to evaluate performance of the VC-ISP system. 

\subsection{Cellular And VC-ISP Simulator}
\label{subsec:cvsvc}

We simulated a 3-level VC-ISP hierarchy in Python, to compare and contrast performance with conventional cellular networks in the case of random failure events. The first level in our hierarchy was the cloud controller, which is assumed to never fail. The second and third levels are regular nodes (VCNs). 

{\em Simulation Procedure:} The nodes at second level contribute 60\% of the simulated traffic, while the nodes at third level makeup the remaining 40\%. At periodic time intervals, random failure events occur, comprising of link failures between the two nodal levels or link failures between a node and the cloud. Thus, we are able to estimate the traffic that is dropped because of the corresponding failure event and the component it affects. Using Monte Carlo simulations, we are able to plot the average amount of failed/dropped traffic. This experiment is repeated after varying the number of nodes in various levels of the hierarchy. In the case of conventional cellular networks, it is assumed that the serving gateways and packet gateways are located in the cloud, and that the traffic is a value proportional to the total number of nodes. 

In addition to this simulator, we also implemented the two identity management models to compare them across the time taken to converge in issuing identities with different volumes of user activity. We have created a 10-node AWS deployment with nodes in different geographic localities to simulate multiple cloud controllers. The locations of the AWS datacenters include California, Oregon, Virginia, Singapore, Frankfurt, Sydney, Tokyo, Ireland and Sao Paulo. Each of the nodes run a Python-based HTTP server, and HTTP \texttt{GET} requests are used to simulate inter-node communication. 

\subsection{Three Node VC-ISP}
\label{subsec:3node}

We built and evaluated a VC-ISP with three nodes, located in Kumawu (Ghana), New York City (USA ) and Abu Dhabi (UAE). Furthermore we also built a relatively stable backhaul for the node in Ghana using signal boosters. The cloud component of all applications was implemented on an AWS node located in Frankfurt (Germany). The implementation details of each of the aforementioned components is given in greater detail below.

\noindent{\bf 1. BTS Nodes:} We used two hardware platforms as Base Transceiver Station (BTS) nodes. The first was a 1 Watt RapidCell from Range Networks \cite{range}, and the second was a 10 mWatt USRP B100 from Ettus Research. We positioned one USRP B100 BTS in Abu Dhabi, another in New York, and finally positioned the RapidCell in Kumawu. We modified the OpenBTS software, specifically the peering module to enable our implementation of white space detection and usage. This modified version of OpenBTS was run on all the BTSs along with smqueue and sipauthserve which deal with SMS and user authentication respectively. Freeswitch PBX was used for routing calls, messages and data. 

We placed a PC next to the BTS setup and refer to it as the local server. This PC hosted the local component of all the applications we support. It is important to note that even without this PC, the OpenBTS combined with smqueue, sipauthserve and Freeswitch is able to provide the functionality of a VCN. As a local component of the IVR application, we deployed an Asterisk PBX on local server to which all the calls coming on IVR system were routed. The local server was also running an HTTP-based marketplace and the mapping server, the respective local components of the corresponding applications. All these applications were written in Python.

\noindent{\bf 2. Cloud Controller:} We use an AWS EC2 instance hosted in Frankfurt as the location is roughly equidistant from New York, Abu Dhabi and Kumawu. The instance had a memory of 1 GiB and was allocated a single vCPU. Our EC2 instance was running Ubuntu 14.04, and all application support on the cloud is written using Python. The specs of the instance suffice for application support as the require minimal processing. The instance is primarily used as a persistent store.

\noindent{\bf 3. Applications:} We conducted experiments with our three applications running simultaneously to ensure simultaneous liveliness in primitive functionality. For the purposes of discussion, let us focus on the marketplace application. To test its local and cloud component, we built an Android application that enables phones to automatically \texttt{SELL} and \texttt{BUY} items in a periodic manner. We had 4 phones sending \texttt{SELL} messages and 3 phones sending \texttt{BUY} and \texttt{SEARCH} messages. 5 of the 7 phones were connected to the BTS in Ghana and the others were connected to the BTS in New York. Calls made manually and script generated data were both routed to the server to increase its processing. 

%We repeated our experiments several times and made the following high level observations.
%a) Neither the local server nor cloud server crashed or reset the connection;
%b) The backhaul link did not break down;
%c) Rapidcell and the USRP node in New York were responsive and sms replies came in a few minutes.

\noindent{\bf 4. Directional Cellular Backhaul:} We built and evaluated a directional cellular backhaul in Ghana and used that to connect the Ghana VCN to the IP network. We used Phonetone K3B0918217CLB kit which comprised of a 10 db directional receiving antenna, 9db indoor panel antenna and 70db analogue booster able to work in 900/1800/2100 MHz GSM bands. In New York, we used a zBoost ZB545X signal booster and a zBoost CANT-0042 wide band directional receiving antenna. 

%This booster had the capability of boosting the 3G signal which in US is delivered in the 1900 MHz GSM band. We wanted to use a 3G band booster because we wanted to compare it to booster performance in Ghana where mostly 3G coverage is available.

\subsection{White Spaces-Based Deployment}

%We deployed our whitespaces solution by modifying the OpenBTS code base. OpenBTS has a peering component that connects to the nearby base stations whose IPs are given in configuration setting of the base station. It exchanges packets with the other base stations and asks them the channels they are operating on. These channels are later set in the layer 2 GSMTAP messages exchanged between the base station and the mobile devices. The base stations send out channels on which neighbors are running and instructs the phones to scan the energy on these channels. The phones scan the energy and report the energy back to the base station in the form of \texttt{Measurement Report} packets.

We modified the peering component of OpenBTS to add duplicate IPs as neighbors. We then intercept the messages being sent to the peers and bypass the checks to update the neighbors database with fake neighboring base stations. We read the channels to scan from a file on disk that has been populated by our Measurement Report scanner. Once the fake neighbors are successfully set, we wait for the base station to send the new neighbor list out to the phones. Once the phones get the neighbor list they start reporting the energy on the fake neighbor channels. We constantly run \texttt{tcpdump} on the GSMTAP port and intercept all the packets being exchanged between phones and the base stations. For this we modify the code base~\cite{gsmws_code} available by the developers of gsmws~\cite{gsmws}. We present the detected white spaces over the period of one week in the 120 channels in the GSM-900 band and present the results in the next section. We also developed an android application that was given to some volunteer users. This application helped us gather reports frequently by sending SMS between volunteers and the base station. More communication by phones means regular reports are exchanged between phones. We extrapolate from data that our solution of having volunteers outperforms NGSM in the next section. 

%We also designate some phones as volunteers in the area and install our android based application in them that keeps sending sms in the background which consequently generate a constant stream of Measurement Report packets. Based on the reports data we collected with and without the volunteers we estimated the rates at which measurement reports are received at the base station with and without volunteers. We then also calculated the number of packets it takes in the worst case to identify the energy of the channel based on our data points. This is important because users(phones) are constantly moving and can take some time to report the channels back. This can result in several packets reporting zero energy on a channel that is potentially being used by someone else. We then used this knowledge to simulate how long it takes NGSM to whitespaces among a particular set of channels.  We present the results for this in the next section.
%We periodically parse all of the Measurement Report packets and populate a database containing the average, maximum and minimum reported energy on each scanned channel. If we do not receive energy reading for a channel we assume that the channel is not being used. To make sure that Measurement Reports are regularly exchanged between the base station and phones we developed an application that calls and texts another mobile device constantly. This helps us ensure that we keep receiving periodical reports from mobile devices. This applcation was developed in Android and was ran on multiple phones while doing whitespaces measurements. We show the results of our whitespaces deployment in the next section.


==> content/8-a_eval.tex <==
\section{Evaluation} 
\label{sec:eval}

\begin{figure}
\centering
%\begin{subfigure}[b]{0.3\textwidth}
   \includegraphics[scale=0.3]{figures/call-gca-cca-constant-failure-rate}
	%\label{server_client_a}
%\end{subfigure}
\caption{VCISP vs Conventional Cellular}
\label{vcisp_vs_cellular}
\end{figure}

\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
Metric & Definition \\
\hline
 VCE & VC-ISP Call Error \\
 CCE & Cellular Call Error \\
 VSE & VC-ISP SMS Error \\
 CSE & Cellular SMS Error \\
 VDE & VC-ISP Data Error \\
 CDE & Cellular Data Error \\
\hline
\end{tabular}
\caption{Metrics used in Figure~\ref{vcisp_vs_cellular} and their definitions. }
\label{tab1}
\end{table}


In this section we evaluate the performance of VC-ISP along four dimensions, namely: (a) performance of the naming and addressing subsystem in comparison with conventional cellular, (b) application quality and reliability, (c) performance of the white spaces detection subsystem, and (d) performance of the signal booster based backhaul.

\subsection{VC-ISP vs Cellular}

\begin{figure}
\centering
%\begin{subfigure}[b]{0.3\textwidth}
   \includegraphics[scale=0.3]{figures/box_combined}
	%\label{server_client_a}
%\end{subfigure}
\caption{Latency for issuing identities: Single server vs 10-node DHT}
\label{server_client}
\end{figure}

We discuss the results of the implementation in \S \ref{subsec:cvsvc}, where figure~\ref{vcisp_vs_cellular} contrasts VC-ISP and conventional cellular networks. The latter have serving gateways and packet gateways far from the actual base stations. Once the link to the base station is down, they become useless. In the analogous case, while the link between the cloud controller and the node is down, the node continues to provide local access. Therefore VCE, VSE and VDE values are always lower than their corresponding cellular counterparts. This general trend suggests that lower error rates are a consequence of a larger number of sites and users. This increases the total calls, ergo reducing the impact of a single failure (simulated within each time interval).

\noindent{\bf Identity Management:} The box and whisker plot in figure~\ref{server_client} compares the client-server model to the DHT-based model in terms of issuing a new global identity to a user. Issuing a new global identity entails issuing a serialized HTTP query to Nexmo. In the DHT-based model, the requests were generated by multiple processes in the node at Frankfurt while other nodes were responsible for processing the request and forwarding it to Nexmo. A synthetic hash function evenly divides the requests to the corresponding nodes that process it, without any location bias. In the client-server model, similarly generated requests were both initiated and responded to by the local host server on the Frankfurt node. It can be seen that the DHT outperforms the single server, even when the number of users is low. This is true as the cumulative processing power in a 10-node DHT exceeds that of a single node server.  

%Figure~\ref{server_client_a} shows the box and whisker plot for the end to end latency experienced by each new identity request. The x-axis shows the number of requests each of the 5 base stations is sending to the server and y-axis shows the time taken in seconds by the single server to process the identity request. It can be seen that as the number of requests increases, the time taken for server to process the requests also increases almost linearly. Similarly Figure~\ref{server_client_b} shows how the failures increase with the increase in users at base each base station. It shows three kinds of failures: Operation Failure, Connection Resets by server, and time outs. While the latter two are caused by network, it is important to see that the server data store is a significant source of contention because the operation failure happens when the data store can not handle consistency. 

\subsection{Service Quality and Reliability}

\begin{figure}
\centering
\begin{subfigure}[b]{0.23\textwidth}
   \includegraphics[scale=0.16]{figures/cdf_sms_times_rapid}
	\caption{Ghana}
	\label{ghana_cdf}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
	\includegraphics[scale=0.16]{figures/cdf_sms_times_lappy}
	\caption{New York}
	\label{ny_cdf}	
\end{subfigure}
\caption{CDF of time it takes for the different functions in the Marketplace application}
\label{cdf}
\end{figure}
\begin{figure}
\centering
\begin{subfigure}[b]{0.23\textwidth}
   \includegraphics[scale=0.16]{figures/cdf_sms_vs_file_post_times_lappy}
	\caption{}
	\label{_cdf}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
	\includegraphics[scale=0.16]{figures/post_complete_times_rapid}
	\caption{}
	\label{_queue}	
\end{subfigure}
\caption{CDF of time taken for the different functions in the marketplace application}
\label{smsvsfile}
\end{figure}
%
%\begin{figure}
%\centering
%
%        \includegraphics[scale=0.2]
%
%\caption{Performance of FASTPUT primitives for different kinds of data:sms vs file}
%\label{smsvsfile}
%\end{figure}

We report the performance of the marketplace application in Figure~\ref{cdf}. The graph above shows the end-to-end latency between the local server and cloud controller for the \texttt{BUY},\texttt{SELL} and \texttt{SEARCH} operations. It is important to recall that the \texttt{SELL} operation translates to the \texttt{SLOWPUT} primitive, while \texttt{BUY} and \texttt{SEARCH} translate to \texttt{FASTGET} and \texttt{FASTSEARCH} primitives respectively. It can be observed in Figure~\ref{ghana_cdf} that \texttt{BUY},\texttt{SELL} and \texttt{SEARCH} operations cause nearly the same end-to-end latency. However in Figure~\ref{ny_cdf}, there is a clear distinction between the performance of \texttt{SELL}, compared to \texttt{BUY} and \texttt{SEARCH}. This is expected because \texttt{SELL} requests are queued and processed in a lazy manner. This distinction is not visible in Figure~\ref{ghana_cdf} as that the bandwidth between cloud and local server is low, consequently increasing latency for both \texttt{SELL} and \texttt{BUY}.

\noindent{\em SMS or File?} Files are typically produced by voice-based or sensing-based applications. Figure~\ref{_cdf} shows the CDF of time it takes for different \texttt{SLOWPUT} requests on the New York-based VCN. Figure~\ref{_queue} shows the queue and how requests are processed for the \texttt{SLOWPUT} primitive for the VCN in Ghana. Figure~\ref{smsvsfile} shows that SMS-based applications will work faster than the file based applications as they are smaller than files. It also shows that file based applications can slow down the SMS-based applications. This is true as both are placed in a common queue for processing, and servicing larger files is more time consuming than servicing smaller SMSs.

\noindent{\em Backhaul Performance:} Using the boosted backhaul, we are able to produce a signal gain of approximately 20 Db in New York. In Ghana, we were able to capture the 3G signal and improve bandwidth significantly. In Figure~\ref{airtel} and Figure~\ref{att} we present the performance of the signal booster based backhaul in New York and Ghana, where the bandwidth gain in TCP and packet loss and jitter improvement in the case of UDP (both measured using \texttt{iperf}) is plotted against trial numbers. The bracket next to each point in the graph shows the average measured \texttt{RSSI} value. This value was measured using Android phones that utilized the boosted backhaul to the BTS node.

\begin{figure}
\centering
\begin{subfigure}[b]{0.23\textwidth}
       \includegraphics[scale=0.22]{figures/airtel_udp_graph}
	\caption{UDP}
	\label{bandwidth_udp}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
       \includegraphics[scale=0.22]{figures/airtel_tcp_graph}
	\caption{TCP}
	\label{bandwidth_tcp}
\end{subfigure}
\caption{Performance of Airtel connection with and without boosted backhaul}
\label{airtel}
\end{figure}

%\begin{figure}
%\centering
%\begin{subfigure}[b]{0.24\textwidth}
%
%        \includegraphics[scale=0.15]{udp}
%\end{subfigure}
%\begin{subfigure}[b]{0.24\textwidth}
%
%        \includegraphics[scale=0.15]{tcp}
%
%\end{subfigure}
%\caption{Performance of AT\&T in New York city with and without backhaul}
%\label{att}
%\end{figure}

The effect of signal boosting Airtel is evident in Figure~\ref{airtel}; we were able to change the transmission rates from EDGE (denoted by E in graph) to that of HSDPA (denoted by H in graph) by capturing the weak 3G signal available in the area. By upgrading, we were able to get significantly more bandwidth as reported by Figure \ref{bandwidth_tcp}. We also reduced the packet loss rate and jitter in UDP as reported by Figure~\ref{bandwidth_udp}. For the New York signal booster results reported in Figure~\ref{att} we observe a significant increase the bandwidth in TCP  due to the signal boosters and we also observe a decrease in packet drop rate in UDP. However UDP jitter increases with the use of a signal booster but the overall gains observed for UDP and TCP flows are significant.


\begin{figure}
\centering
%\begin{subfigure}{0.5\columnwidth}
       \includegraphics[scale=0.3]{figures/Whitespaces_1st_week}
%\end{subfigure}
\caption{Used and unused channels over one week in Kumawu Ghana.}
\label{spectrum}
\end{figure}


\subsection{Whitespaces Performence}
\begin{figure}
\centering
\begin{subfigure}[b]{0.23\textwidth}
       \includegraphics[scale=0.22]{figures/aa45}
	\caption{Energy reported}
	\label{channel_value}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
       \includegraphics[scale=0.23]{figures/ab45}
	\caption{Frequency of reports}
	\label{channel_frequency}
\end{subfigure}
\caption{Channel energy as reported by various measurement reports and frequency of reports at a 5 min granularity.}
\label{channel_info}
\end{figure}

We implemented our whitespaces solution as mentioned above. In Figure~\ref{spectrum} we show the results of our measurements. We show the unused and used channels in the P-GSM-900 spectrum which is made up of 124 channels starting from arfcn 1 and ending at arfcn 124. We choose this spectrum because this was the spectrum in which our device was operating. The results highlight a few important finding: GSM whitespaces are indeed available in rural areas and can be exploited by using the mechanism we explained above.
\begin{figure}
\centering
\begin{subfigure}[b]{0.23\textwidth}
   \includegraphics[scale=0.22]{figures/ngsm_simulation_0point1}
	\caption{}
	\label{0point1}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
	\includegraphics[scale=0.22]{figures/ngsm_simulation_0point2}
	\caption{}
	\label{0point2}	
\end{subfigure}
\caption{CDF of time it takes for the different functions in the Marketplace application}
\label{ngsm_vs_us}
\end{figure}

Figure~\ref{channel_value} shows in chronological order the various readings over the period of approximately 4 hours. Figure~\ref{channel_frequency} shows for the same channel the plot of how many reports were received every 5 minutes. These two graphs highlight the fact that there is a constant need for sensing the channel because even for such channels which are clearly being used by a neighboring base station there are a significant number of reports telling that the energy on channel is zero (the horizontal line at y=0 in Figure~\ref{channel_value}. While analyzing other channels we observed that it can take hundreds of zero energy packets and several minutes before a packet reporting a positive energy on a channel is received.  There can be many possible reasons for this. One possible reason is that the overlap radius is very small and the mobile device is only able to see energy on a channel for very small amount of time. Because of this we argue for having some phones as volunteers in the area who install our android based application in them. The application keeps sending sms in the background to other volunteers and the base station. This results in a rather constant stream of Measurement Report packets. Similarly we increase the radius of coverage (transmission power) of our base station slowly if we have no knowledge of the available channels in the area. So that we can get some time to sense the channel and identify even the most weak interfering signals. 
Based on the reports data we collected with and without the volunteers we estimated the rates at which measurement reports are received at the base station with and without volunteers. We then also calculated the number of packets it takes in the worst case to identify the energy of the channel based on our data points. This is important because users(phones) are constantly moving and can take some time to report the channels back. This can result in several packets reporting zero energy on a channel that is potentially being used by someone else. We then use this knowledge to simulate how long it takes NGSM~\cite{gsmws} to discover whitespaces among a particular set of channels as compared to how much time our solution takes with the help of volunteers. We present the results for this in Figure~\ref{ngsm_vs_us}. The x-axis of Figure~\ref{0point1} and Figure~\ref{0point2} show the number of active users. The number of channels scanned at each data point is the same as the number of users.  The y-axis shows the number of minutes it takes for us to scan the channels. It can be seen that our volunteer based method performs better than NGSM where there are no volunteers. The volunteer to user is 0.1 in Figure~\ref{0point1} and 0.2 in Figure~\ref{0point2}.  




==> content/abstract.tex <==
\begin{abstract}

Achieving reliable rural cellular connectivity is a challenging problem due to several real-world factors: lack of economic incentives for telecom providers, high deployment and maintenance costs, low purchasing power, poor and unreliable power infrastructure, poor backhaul support and lack of ground expertise. This paper proposes the design, implementation and deployment of {\em Virtual Cellular ISPs (VC-ISP)}, a new ground-up cellular network architecture that enables third-party vendors to offer cellular coverage and mobile services in rural areas in an extensible manner. Unlike the conventional monolithic cellular network architecture, the VC-ISP model enables a distributed (and potentially disjoint) collection of open, programmable cellular base stations combined with directional boosted backhauls to collectively provide a gamut of both conventional cellular services and new forms of distributed edge services. VC-ISPs can provide reliable and intermittency-aware network services with graceful recovery from failures under harsh real-world conditions. VC-ISP offers new application primitives to support different types of intermittency-aware distributed mobile edge services including P2P transactions, voice-based social media applications, and distributed mobile sensing applications. Using a participatory sensing white spaces approach, a VC-ISP can both co-exist with other conventional cellular networks and other VC-ISPs. We demonstrate the practical viability of the VC-ISP model using a real-world 3-node VC-ISP deployment including a solar-powered cell tower installation in rural Ghana and additional emulation experiments under controlled environments. The Ghana installation also supports different forms of new mobile services used within the rural community.

\end{abstract}


==> content/conclusion.tex <==
\section{Conclusion}

==> content/deployment.tex <==
\section{Deployment}
\label{sec:deployment}

Before delving into a greater depth of technicality, we first describe our real-world VC-ISP deployment. This deployment utilized 3 VCNs, located in New York (USA), Kumawu (Ghana) and Abu Dhabi (UAE).  All nodes run a modified version of OpenBTS \textcolor{red}{modified to reflect what?}. The node in Ghana had transmission power of 1 Watt, while the nodes in New York and Abu Dhabi where much smaller. Our VC-ISP supported primitives for deploying SMS, call and data based applications. These include an SMS-based marketplace, an interactive voice response (IVR) based social network application, and a data sensing application. All the applications were hosted at the edge i.e. at node + local servers, and nodes communicated with each other using a smart bandwidth management layer to effectively utilize the available capacity. We describe the VCN setup in Kumawu in greater detail. 

\subsection{VCN At Kumawu}

\begin{figure}
\centering
        \includegraphics[scale=0.2]{PowerGraph.pdf}

\caption{State of battery attached to solar panels, corresponding to weather conditions while running the base station over a week}
\label{powergraph}
\end{figure}

\begin{figure}
\centering

        \includegraphics[scale=0.2]{picture.pdf}

\caption{The picture of deployment, showing the directional backhaul antenna, omni-directional base station antenna and solar panels}
\label{deployment}
\end{figure}

{\bf Background:} Kumawu is a small neighborhood 2 hours away from Kumasi, one of the largest cities in Ghana. The two major cellular providers in Kumawu are MTN and Airtel. Based on our measurements, we concluded that MTN had reasonable coverage in most parts of Kumawu, but not in the peripheries. On the other hand, Airtel had coverage (including 3G) only till the mid town, only 2.5G services were available from Airtel beyond that point. 

{\bf Deployment Specifications:} The node at Kumawu was deployed at the edge of existing coverage i.e. approximately 500 meters away from Airtel's 3G coverage boundary. We constructed a cheap and low-cost backhaul for our VCN using an omni-directional receiving antenna. This enabled us to catch the weak 3G signal available 500 meters away, and redirect this weak signal to an analogue signal repeater to amplify. We then pass the signal to an indoor antenna where a phone is used to receive the signal and provide tethered internet to the earlier defined local server. This server is responsible for communicating with the cloud controller and other VCNs. Figure~\ref{deployment} shows various components of our deployment in Ghana, including the directional antenna. In \S , we present evaluation of our DIY backhaul. 

Our base station unit had a 1 Watt transmission power and was manufactured by Range Wireless \cite{range}. The coverage range of base station is dependent on several environmental factors, with the advertised coverage radius of 1 to 7 kilometers. Our area of deployment was hilly and we mounted the antenna relatively low, therefore in our experiments we measured coverage diameter was over 1 kilometer. 

{\bf Preliminary Observations:} We made the following assumptions with regards to the power consumption and mobility of our deployment.


\begin{itemize}
\itemsep-0.23em

\item In spite of having a coverage range comparable to cellular base stations in metropolitan areas, our base station had reduced power consumption. The low power profile of the apparatus used enabled us to power the base station using solar panels of capacity 1 KW. Figure~\ref{powergraph} shows the state of battery attached to solar panels and the corresponding weather conditions across that week. % while the base station was solar powered. 
As expected, the rate at which the battery charges is highly dependent on the availability of sunlight. This rate, however, is moderate even in cloudy and overcast conditions. Though failures are expected if the overcast conditions persist, the intermittent grid power can be used that to recharge the battery in such cases. The power consumption of the base station itself is a few Watts \textcolor{red}{how many exactly?}, while the complete setup, consisting of signal booster, local server and base stations never exceeded 300 Watts.  

%It is worth mentioning that the biggest part of our deployment were the solar panels and the omni-directional base station antenna. 
\item It can be seen in Figure~\ref{deployment} that the omni-directional antenna and solar panels are not excessively large, unlike those at a few conventional base station sites. Additionally, these solar panels are mounted atop a trolley to provide mobility. Thus, these deployments can easily be taken to rural areas and quickly deployed. These portable, mobile deployments can also be very useful in case of natural disasters \cite{rescue_base_station}. 
\end{itemize}






==> content/relatedwork.tex <==
\section{Related Work}

{\bf Software-based microcells:} Universal service obligations have been pushed by many countries to facilitate the expansion of communication into rural areas. 
%In this model money collected from levying extra tax is used to subsidize providers to expand into rural areas. But these methods have not worked: A survey of 64 USFs showed that most remain inefficient and ineffective with more than USD 11 billion waiting to be disbursed between them~\cite{gsma_report}. The use of competition based methods\cite{chone2002allocating,weller1999auctions} but the reality on ground is unchanged and millions of people live without cellular access. As a paralell to the above model of pushing nationwide cellular companies to expand, there is a history of small-scale cooperative or locally owned telephony networks. 
In parallel recent advances in hardware and open-source software has made available inexpensive cellular equipment broadly accessible. For example, OpenBTS is an open-source GSM base transceiver station (BTS) implementation which has enabled a wide range of projects aimed towards building small-scale VCNs. Heimerl et al.\cite{kurtis_ictd} demonstrated the viability of independently run, locally operated cellular networks. Similarly, Rhizomatica\cite{rhizo} has deployed several community-run cellular networks in Oaxaca, Mexico with a short-term experimental spectrum license. Zheleva et al.~\cite{zheleva} deployed a similar system for purely local communications in Zambia. %Except for the Rhizomatica deployments all others including our deployment in Ghana operate without licenses.

%\textbf{Software Defined Networks:}
%SDNs were first introduced by the white-paper called OpenFlow\cite{openflow} but many argue that the journey towards seperation of control plane from dataplane began with the 4D project\cite{rcp,4d,rexford}. Sane\cite{sane} and Ethane\cite{ethane} were the first systems developed using the concepts introduced by OpenFlow\cite{openflow}. This was soon followed by NOX\cite{nox} which was the first opensource implimentation of an SDN controller anyone could experiment with. In paralell to NOX, Maestro\cite{maestro} was developed but NOX remained the first controller to be made opensource.
%Many other OpenFlow controllers have been released since NOX. The popular ones are Beacon\cite{beacon} and Onix\cite{onix}. Orthoganal to controllers Mininet\cite{mininet} was developed in order to enable rapid prototyping for SDN ideas on a single or few machines. In paralell to the controllers various systems to facilitate enterprises were also developed. People have focused on the networks in the context of data centers\cite{difane,nv,data-center1,flowvisor} and there has only been relatively very little focus on SDN in WANs and Google's effort to manage their data-centers using and SDN controller is the most prominent work in this space\cite{b4}.
%SDNs have been provably effective in data-center setting but they have not been designed for networks that might have high latency and low bandwidth. In this paper we try to highlight the limitations of SDNs in one such network architecture. We also give our vision which is in some ways similar to Difane\cite{difane} as we try to reduce the burden on the central controller and try to make as many decisions as possible in the data plane. We are different from Difane because Difane was built for a data-center environment in which the all the routers are controlled by a central controller, which is not the case in our network as we rely on internet routers.

\textbf{Backhauls and rural mesh networks:} The design of VC-ISP builds upon a large body of work across rural wireless networks including Fractel~\cite{fractel}, Digital Gangetic Plains~\cite{inside_out,gangetic,2P}, WiLDNet~\cite{wildnet,beyond}. There has been immense around design of various different Line of Sight(LOS) and Non Line of Sight Cellular(NLOS) backhauls~\cite{tarana,kumu}.   

\textbf{Cognitive Radio and GSM whitespaces:} The literature on cognitive radio, whitespaces, and dynamic spectrum sharing is vast; while most work in the space focuses on TV whitespaces (TVWS), our work is more closely related to work on re-use of cellular spectrum. Sankaranarayanan et al.~\cite{sankaranarayanan2005bandwidth} propose reusing timeslots in a GSM cell for adhoc networks during periods when the GSM cell is lightly utilized. Buddhikot et al.~\cite{buddhikot2009ultra} describe a system for indoor femtocells to dynamically share spectrum with incumbent carriers by operating over ultra wide bands. Yin et al.~\cite{yin_beijing} proposes a similar system and provides measurement results which indicate that unused spectrum (i.e., whitespace) exists even in a dense, urban environment (Beijing). The assumption in the community, however, seems to be that cellular spectrum is efficiently used and that finding GSM whitespace is challenging. In contrast to these, we focus on reusing GSM whitespaces to provide GSM service by means of macrocells. The only work that recycles GSM whitespaces for reuse by a VCN is NGSM~\cite{gsmws}. We have already highlighted how our approach for doing GSM whitespaces builds on top of NGSM and performs better. 


\textbf{Intermittency aware networks:} VC-ISP also significantly benefits from prior work on Delay Tolerant Networks~\cite{dtn_routing,seth2006lcc}.  One of the first real world DTN deployments was DakNet which provides low-cost digital
communication to rural areas using physical transportation
links~\cite{pentland2004daknet}.  There have been several routing
DTN-based routing algorithms like Encounter based
routing~\cite{nelson2009encounter} and MobySpace~\cite{leguay2005evaluating}. \cite{burgess2006maxprop, juang2002energy, chaintreau2007impact} are other works that use DTN centric ``store and forward'' algorithms to progressively forward
messages until they reach their destination.
The intermittency awareness abstraction of VC-ISP is fundamentally
different from the traditional DTN abstractions since VC-ISP is
primarily tailored and designed for the cellular network context and primarily focuses on higher application-centric ``store and forward'' abstractions; the DTN routes for VC-ISP messages are preset by the network structure which changes infrequently. 




==> content/whitespaces.tex <==
%\section{Our GSM Whitespaces Solution}
\section{Detecting Whitespaces}	
\label{sec:gsm}

%VCN based model of cellular networks has been shown to work in areas that have low population density~\cite{kurtis_ictd,zheleva,rhizo}.

Wireless spectrum is auctioned on a regular basis to large telecommunication organizations. Commercial networks deploy multiple cells covering large, contiguous areas. Though they purchase slivers of the available spectrum, majority of these slivers remain unused in developing regions. These unused bands of spectrum are collectively called GSM whitespaces. The existence of these whitespaces has been proved for a remote area in Indonesia and a system has been built to operate without interfering with the licensed providers \cite{gsmws}. Thus, VCNs largely operate using these whitespaces, without spectrum licenses in localized communities where cellular connectivity is limited. 

{\em Nomadic GSM:} Proposed by Hassan et al. \cite{gsmws}, this scheme uses handsets to continuously measure spectrum occupancy and report measurements back to their serving cell. The authors claim that their system safely uses unused licensed spectrum without requiring cooperation or participation from existing license holders. NGSM takes advantage of the fact that GSM handsets continually measure spectrum occupancy in their proximity and report these measurements to their serving cell, ergo mitigating the practical impact of the hidden node problem caused by client side interference. However, NGSM has the following limitations:
%In our deployment we try to improve upon the following limitations in NGSM: 

\begin{enumerate}
\itemsep-0.23em

\item The secondary base station begins to transmit at full power on a randomly chosen Absolute Radio Frequency channel Number (ARFCN) before any sensing is done. This can lead to interference with a primary base station operating in that ARFCN. 

\item In the scenario where there is no call or SMS between users, the measurement reports to the serving cell become infrequent. This is often the case in low population density regions. This can lead to delayed readings, which can further lead to wrongfully using a channel that interferes with a primary license holder. 

\item The system requires two base stations in the same location, so that active calls in the primary can be moved to the secondary when the primary is collapsed. This requirement of a secondary is often cumbersome and financially unfeasible.  

\end{enumerate}

The GSM whitespaces detection mechanism we use is a hybrid of sensing and database approaches, similar to NGSM, addressing the aforementioned concerns. The first limitation of NGSM is mitigated by increasing transmission power periodically to slowly expand coverage. This is done while simultaneously sensing for used channels among a list of safe channels. In this manner, there is no need to have any prior knowledge of ARFCN usage. Thus, a small software-defined base station can be installed at any location without examining the spectrum prior, because any interference caused will be at a much smaller radius than compared to a base station transmitting at full power. The second limitation is addressed using a mobile application that periodically makes calls and sends messages to the base station. This ensures periodicity, ergo frequency in measurement reports. \textcolor{red}{what about the economic feasibility of this aspect? if each call costs x dollars, what will the cost be of making 100 such calls?} If a few volunteers in the community run this application, the cost associated with it can be divided across all community members to ensure a nominal increase in their payments. Finally, we do not expect the presence of two different base stations, and instead wait for the connected calls to complete in case it is time to shift to a different safe channel. \textcolor{red}{what is the difference in latency between their approach and yours? i.e is there any user perceived delay in your method which is avoided in theirs? if so, we need to write about it here for completeness.} 




==> plantext_talal.tex <==
Talal: I think the paper should be titled: "Experiences deploying extreme edge services as an alternative to core based services". 

S1: Introduction

I agree with Varun below. The pitch is going to be like this. Rural environments are harsh for a variety of reasons, reasons are already listed in intro. Makes providing conventional services hard. We need to go into more detail with respect to how services are being deployed. 
We need to end intro with our various components that help us build edge based services. These components are going to be Backhaul, whitespaces, power and then the services itself is built on top of these. The naming addressing stuff going out. This is going to go in the VC-ISP pitch for GAIA. 


S2: Related Works
Related works is mostly written. We can just bring it up and then see what are the references that are missing. 

S3: Design
Design of various things discussed in intro. 
Architecture, backhaul, whitespaces and power. 

S4: primitives and services

explanation as to why edge services are key to functioning successfully in these regions; various components that are requiered to provides these services
a. seperation of applications into local and cloud components with synchronization primitives between the two
b. CAP specification i.e the battle between C,A,P as and when needed
c. how this seperation+specification makes sense, explicitly in this kind of harsh environment; in this absence of any infrastructural support

S5: Implementation

S6: Evaluation and Discussion

